Language Modelling as a Multi-Task Problem

In this paper, we propose to study language modelling as a multi-task problem, bringing together three strands of research: multi-task learning, linguistics, and interpretability. Based on hypotheses derived from linguistic theory, we investigate whether language models adhere to learning principles of multi-task learning during training. To showcase the idea, we analyse the generalisation behaviour of language models as they learn the linguistic concept of Negative Polarity Items (NPIs). Our experiments demonstrate that a multi-task setting naturally emerges within the objective of the more general task of language modelling.We argue that this insight is valuable for multi-task learning, linguistics and interpretability research and can lead to exciting new findings in all three domains.

==> notes <==
- second sentence is grammatically incorrect
- 028 However, current MTLP implementations fall back on... --> this needs to be a more impersonal sentence, something like "To decide on ... arbitrary decisions and etc are necessary", then an example to illustrate this
- 032 "This is convenient from an engineers ..." --> Better to state that also for engineers this is inconvenient (they have to choose hyperparams etc, make a lot of arbitrary decisions, this is annoying). So, we have two-fold problem:
    - inconvenient for researchers that work on MTL
    - stands in the way of understanding MTL in neural models, because we don't know if conclusions are due to unrealistic scenarios (tasks and curriculum) or hyperparam choices.

Put more weight on the second: "This is a hassle for researchers working on MTL (having to make all kinds of arbitrary decisions) but, more importantly, stands in the way of understanding the extent to which NNs can do multitask learning 

Implied here is the two-fold advantage (which perhaps we don't need to make explicit):
- We can study to what extent neural networks can do multitask learning: can they accommodate different tasks, pick up on their similarities and benefit from them?
- We can learn from this natural setup where many choices are already taken and transfer this knowledge to other scenarios where it might be necessary to consider more unrealistic combinations of tasks --> transfer knowledge about curriculum of what can learn from what, for instance).

Here, we propose to -- instead of generating artificial scenarios to study MTL -- study MTL in the more natural setting of language modelling, by exploiting the fact that language modelling itself can be seen as a compilation of many different smaller tasks.
*Give an example*
All of these construction rules have to be optimised in parallel.
Language modelling is in that sense a \textit{natural} MTL problem, with a naturally given sub-task hierarchy. (I like this "subtask hierarchy, but it should be mentioned already earlier for the reader to understand this)

Studying language modelling as a multitask problem has a multitude of advantages.
First,
- 


